A Low Complexity Detection Algorithm Based on Alternating Minimization

In this paper, we propose an algorithm based on the Alternating Minimization technique to solve the uplink massive MIMO detection problem. The proposed algorithm provides a lower complexity compared to the conventional MMSE detection technique, especially when the number of user equipment (UE) antennas is close to the number of base station (BS) antennas. This improvement is obtained without any matrix inversion. Moreover, the algorithm re-formulates the maximum likelihood (ML) detection problem as a sum of convex functions based on decomposing the received vector into multiple vectors. Each vector represents the contribution of one of the transmitted symbols in the received vector. Alternating Minimization is used to solve the new formulated problem in an iterative manner with a closed form solution update in every iteration. Simulation results demonstrate the efficacy of the proposed algorithm in the uplink massive MIMO setting for both coded and uncoded cases

==> sec06_conc.tex <==

%\section{Future work}

\vspace{-0.08in}

\section{Conclusion and Future work}

In this paper, a two-stage LASSO ADMM algorithm for large scale MIMO signal detection is investigated. Numerical results demonstrate the superiority of the proposed algorithm compared to the conventional methods for both coded and uncoded symbols at various QAM modulations. Investigating Multi-Stage LASSO-ADMM is an interesting future work. 
\vspace{-0.150in}
%We are currently investigating Multi-Stage LASSO ADMM Signal Detection Algorithm For Large Scale MIMO where $N$ stages are considered $(N > 2)$. Our preliminary results show further performance improvement when the rounding thresholds are well chosen per stage and for some values of $\lambda$ which interests us to understand in more depth the theory behind choosing these parameters..Finally,  we are working on Multi-Stage Generalized LASSO ADMM Signal Detection Algorithm for Spatial Modulation. In spatial modulation, not only the coefficients are sparse, but also the transmitted symbols since only one or few antennas is/are active at any given time.
